System FR as Foundations for Stainless

We present the design, implementation, and foundation of a verifier for higher-order functional programs with generics and recursive data types. Our system supports proving safety and termination using preconditions, postconditions and assertions. It supports writing proof hints using assertions and recursive calls. To formalize the soundness of the system we introduce System FR, a calculus supporting System F polymorphism, dependent refinement types, and recursive types (including recursion through contravariant positions of function types). Through the use of sized types, System FR supports reasoning about termination of lazy data structures such as streams. We formalize a reducibility argument using the Coq proof assistant and prove the soundness of a type-checker with respect to call-by-value semantics, ensuring type safety and normalization for typeable programs. Our program verifier is implemented as an alternative verification-condition generator for the Stainless tool, which relies on existing SMT-based solver backend for automation. We demonstrate the efficiency of our approach by verifying a collection of higher-order functional programs comprising around 14000 lines of polymorphic higher-order Scala code, including graph search algorithms, basic number theory, monad laws, functional data structures, and assignments from popular Functional Programming MOOCs.

==> figures/fig-badfib.tex <==
%! TEX root = ../main.tex

\begin{figure}

\begin{lstlisting}
def badZipWith[X,Y,Z](f: X $\Rightarrow$ Y $\Rightarrow$ Z, s1: @*\Stream{X}*@, s2: @*\Stream{Y}*@): @*\Stream{Z}*@ =
  fold (
    f (@*\shead{s1}*@) (@*\shead{s2}*@),
    $\lambda$(u: $\tunit$). badZipWith[X,Y,Z](f, @*\stail{(\stail{s1})},\ \stail{(\stail{s2})}*@)
  )

def badFib: $\Stream{\tnat}$ =
  fold(0,
    fold(1,
      $\lambda$(u: $\tunit$). badZipWith[$\tnat$,$\tnat$,$\tnat$](plus, @*\stail{badFib}*@, @*\stail{(\stail{badFib})}*@)
    )
  )
\end{lstlisting}

\caption{A diverging stream}
\end{figure}


==> figures/fig-bodyvisible.tex <==
%! TEX root = ../main.tex

\begin{figure}[htb]

\begin{tabular}{c} % for centering the listing
\begin{lstlisting}
def f(n: $\tnat$): $\tnat$ = {
  decreases(n)

  n match {
    case 0 $\Rightarrow$ 1
    case S(m) $\Rightarrow$ divide(1000,f(m)) + 1
  }
}
\end{lstlisting}
\end{tabular}

\caption{A function that always returns a strictly positive number.}
%   The \lstinline!assert($t_1$) in\ $t_2$! construct is syntactic sugar for
%   $\tite{t_1}{t_2}{\terr}$ and is type checked as such. }
\label{fig:bodyvisible}

\end{figure}


==> figures/fig-constant.tex <==
%! TEX root = ../main.tex

%%%%% UNUSED FILE

\begin{figure}[htb]

\begin{lstlisting}
def constant[X](x: X): @*\Stream{X}*@ = fold (x, $\lambda$(u: $\tunit$). constant[X](x)))
\end{lstlisting}

\caption{An infinite stream repeating {\tt x}}
% \label{fig:constant}

\end{figure}


==> figures/fig-context-embedding.tex <==
%! TEX root = ../main.tex

\begin{figure}
\[
  \begin{array}{l@{}c@{}rcl}
    \lembed\Theta;\Gamma, & y:\trefine{x}{\tau}{p}       & \rembed & = & \embed{\Theta;\Gamma} \wedge \cembed{p[x\mapsto y]}{\Theta;\Gamma,y:\tau}\\
    \lembed\Theta;\Gamma, & p:\tequal{t_1}{t_2}          & \rembed & = & \embed{\Theta;\Gamma} \wedge \cembed{t_1}{\Theta;\Gamma}\simeq\cembed{t_2}{\Theta;\Gamma}\\
    \lembed\Theta;\Gamma ,& f:\tarrow{x}{\tau_1}{\tau_2} & \rembed & = & \embed{\Theta;\Gamma}\\
  \end{array}
\]
\caption{Selection of context embedding rules.}
  \label{fig:context-embedding}
\end{figure}


==> figures/fig-extension.tex <==
%! TEX root = ../main.tex

\begin{figure}

\sidebyside{
    \infer[\textit{(Form Intersection)}]{
        \istype{\Gamma}{\tintersect{\tau_1}{\tau_2}}
    }{
        \istype{\Gamma}{\tau_1} &
        \istype{\Gamma}{\tau_2}
    }
}{
    \infer[\textit{(Form Union)}]{
        \istype{\Gamma}{\tunion{\tau_1}{\tau_2}}
    }{
        \istype{\Gamma}{\tau_1} &
        \istype{\Gamma}{\tau_2}
    }
}

\seprules

\sidebyside
{
    \infer[\textit{(Form Forall)}]{
        \istype{\Gamma}{\tforall{x}{\tau_1}{\tau_2}}
    }{
        \istype{\Gamma}{\tau_1} &
        \istype{\Gamma, x: \tau_1}{\tau_2}
    }
}
{
    \infer[\textit{(Form Top)}]{
        \istype{\Gamma}{\ttop}
    }{
        \iscontext{\Gamma}
    }
} 

\seprules

\sidebyside
{
    \infer[\textit{(Form Exists)}]{
        \istype{\Gamma}{\texists{x}{\tau_1}{\tau_2}}
    }{
        \istype{\Gamma}{\tau_1} &
        \istype{\Gamma, x: \tau_1}{\tau_2}
    }
}
{
    \infer[\textit{(Form Bot)}]{
        \istype{\Gamma}{\tbot}
    }{
        \iscontext{\Gamma}
    }
}
 
 
\seprules

\ 
{
    \infer[\textit{(Form Singleton)}]{
        \istype{\Gamma}{\tsingleton{t}}
    }{
        \iscontext{\Gamma} &
        \fv{t} \subseteq \Gamma
    }
}
 
\seprules

\ 
{
    \infer[\textit{(Intersection Intro)}]{
        \hastype{\Gamma}{t}{\tintersect{\tau_1}{\tau_2}}
    }{
        \hastype{\Gamma}{t}{\tau_1} &
        \hastype{\Gamma}{t}{\tau_2}
    }
}

\seprules

\ 
{
    \infer[\textit{(Union Elim)}]{
        \hastype{\Gamma}{\tlet{z}{\tunion{\tau_1}{\tau_2}}{t}{t'}}{\tau}
    }{
        \hastype{\Gamma}{t}{\tunion{\tau_1}{\tau_2}} &
        \hastype{\Gamma, z: \tau_1}{t'}{\tau} &
        \hastype{\Gamma, z: \tau_2}{t'}{\tau}
    }
}
 
\seprules

\ 
{
    \infer[\textit{(Forall Intro)}]{
        \hastype{\Gamma}{v}{\tforall{x}{\tau_1}{\tau_2}}
    }{
        \isval{v} &
        \hastype{\Gamma, x: \tau_1}{v}{\tau_2}
    } 
}

\seprules

\ 
{
    \infer[\textit{(Exists Elim)}]{
        \hastype{\Gamma}{\tlet{z}{\texists{x}{\tau_1}{\tau_2}}{t}{t'}}{\tau}
    }{
        \hastype{\Gamma}{t}{\texists{x}{\tau_1}{\tau_2}} &
        \hastype{\Gamma, x: \tau_1, z: \tau_2}{t'}{\tau}
    }
}
 
\seprules

\sidebyside
{
    \infer[\textit{(Singleton Intro)}]{
        \hastype{\Gamma}{t_1}{\tsingleton{t_2}}
    }{
        \hastype{\Gamma}{t_1}{\tau} &
        \areequal{\Gamma}{t_1}{t_2}
    }
}
{
    \infer[\textit{(Subtype Singleton)}]{
        \subtype{\Gamma}{\tsingleton{t}}{\tau}
    }{
        \hastype{\Gamma}{t}{\tau}
    }
}
 
\seprules
 
\sidebyside
{
    \infer[\textit{(Subtype Intersection 1)}]{
        \subtype{\Gamma}{\tintersect{\tau_1}{\tau_2}}{\tau_1}
    }{
    }
}
{
    \infer[\textit{(Subtype Intersection 2)}]{
        \subtype{\Gamma}{\tintersect{\tau_1}{\tau_2}}{\tau_2}
    }{
    }
}
 
\seprules

\sidebyside
{
    \infer[\textit{(Subtype Union 1)}]{
        \subtype{\Gamma}{\tau_1}{\tunion{\tau_1}{\tau_2}}
    }{
    }
}
{
    \infer[\textit{(Subtype Union 2)}]{
        \subtype{\Gamma}{\tau_2}{\tunion{\tau_1}{\tau_2}}
    }{
    }
}
 
\seprules
 
\sidebyside
{
    \infer[\textit{(Subtype Forall)}]{
        \subtype{\Gamma}{\tforall{x}{\tau_1}{\tau_2}}{(\tlet{x}{\tau_1}{t}{\tau_2})}
    }{
        \hastype{\Gamma}{t}{\tau_1}
    }
}
{
    \infer[\textit{(Subtype Bot)}]{
        \subtype{\Gamma}{\bot}{\tau}
    }{
        % \istype{\Gamma}{\tau}
    }
}

 
\seprules
 
\sidebyside
{
    \infer[\textit{(Subtype Exists)}]{
        \subtype{\Gamma}{(\tlet{x}{\tau_1}{t}{\tau_2})}{\texists{x}{\tau_1}{\tau_2}}
    }{
        \hastype{\Gamma}{t}{\tau_1}
    }
}
{
    \infer[\textit{(Subtype Top)}]{
        \subtype{\Gamma}{\tau}{\top}
    }{
        % \istype{\Gamma}{\tau}
    }
}


% {
%     \infer[\textit{(Subtype Intersection 2)}]{
%         \subtype{\Gamma}{\tintersect{\tau_1}{\tau_2}}{\tau_2}
%     }{
%     }
% }
 
% \seprules

% \ 
% {
%     \infer[\textit{(Subtype Singleton Identity)}]{
%         \subtype{\Gamma}{\tsingleton{t_1}}{\tsingleton{t_2}}
%     }{
%         \areequal{\Gamma}{t_1}{t_2}
%     }
% }
 
\seprules

\ 
{
    \infer[\textit{(Equal Singleton)}]{
        \areequal{\Gamma}{t_1}{t_2}
    }{
        \hastype{\Gamma}{t_1}{\tsingleton{t_2}}
    }
}

\caption{Rules for intersections, unions, and singleton types.}
\label{fig:extension}
\end{figure}


==> figures/fig-fibonacci.tex <==
%! TEX root = ../main.tex

\begin{figure}[htb]

\begin{center}
\begin{tabular}{c}
% \small
\end{figure}



==> figures/fig-lists.tex <==
%! TEX root = ../main.tex

\begin{figure}

\ 
{
    \infer[\textit{(Form List)}]{
        \istype{\Gamma}{\tlist{\tau}}
    }{
        \istype{\Gamma}{\tau}
    }
}

\seprules

\sidebyside{
    \infer[\textit{(List Intro 1)}]{
        \hastype{\Gamma}{\tnil{\tau}}{\tlist{\tau}}
    }{
        \istype{\Gamma}{\tlist{\tau}}
    }
}{
    \infer[\textit{(List Intro 2)}]{
        \hastype{\Gamma}{\tcons{\tau}{x}{l}}{\tlist{\tau}}
    }{
        \hastype{\Gamma}{x}{\tau} &
        \hastype{\Gamma}{l}{\tlist{\tau}}
    }
}

\seprules
{
    \small
\ 
{
  \infer[\textit{(List Recursion)}]{
    \hastype
      {\Gamma}
      {\trec{l \Rightarrow \tau}{t_l}{t_{nil}}{(x,l',y) \Rightarrow t_{cons}}}
      {\tlet{l}{\tlist{T}}{t_l}{\tau}}
  }{
    \begin{array}{@{}c@{}}
    \istype{\Gamma, l: \tlist{T}}{\tau} \\
    \hastype{\Gamma}{t_l}{\tlist{T}} \qquad
    \hastype{\Gamma}{t_{nil}}{\subst{\tau}{l}{\tnil{T}}} \\
      {\Gamma, 
        x: T, 
        l': \tlist{T}, 
        y: \tau,
        p: \tequal{y}{\trec{n \Rightarrow \tau}{l'}{t_{nil}}{(x,l',y) \Rightarrow t_{cons}}}
      } \vdash
      {t_{cons}}: 
      {\subst{\tau}{n}{\tcons{T}{x}{l'}}}
    \end{array}
  }
}
}

\vspace{1ex}
{
    \small
\ 
{
  \infer[\textit{(List Elim)}]{
    \hastype
      {\Gamma}
      {\tmatch{t_l}{t_{nil}}{(x,l') \Rightarrow t_{cons}}}
      \tau
  }{
    \begin{array}{@{}c@{}}
    % \istype{\Gamma, l: \tlist{T}}{\tau} \\
    \hastype{\Gamma}{t_l}{\tlist{T}} \qquad
    \hastype{\Gamma, p: \tequal{t_l}{\tnil{T}}}{t_{nil}}{\tau} \\
      {\Gamma, 
        x: T, 
        l': \tlist{T}, 
        p: \tequal{t_l}{\tcons{T}{x}{l'}}
      } 
      \vdash {t_{cons}}: \tau 
    \end{array}
  }
}
}

\caption{Rules to add lists in the language.}
\label{fig:lists}

\end{figure}

==> figures/fig-map.tex <==

%! TEX root = ../main.tex

\begin{figure}

\begin{center}
\begin{tabular}{c}
\begin{lstlisting}
def map(l: $\List$, g: $\tnat \rightarrow \tnat$): $\List$ = {
  decreases($\tsize{\tt l}$)
  l match {
    case Nil => Nil
    case x :: xs => g(x) :: map(xs, g)
  }
}
\end{lstlisting}
\end{tabular}
\end{center}

\caption{A map function whose measure is given with {\tt size}.}
\label{fig:map}

\end{figure}

==> figures/fig-measure.tex <==
%! TEX root = ../main.tex

\begin{figure}[htbp]

\hspace{1em}
\begin{minipage}{0.29\textwidth}
\begin{tabular}{c}
\begin{lstlisting}
def f(x: $\tau_1$): $\tau_2$ = {
  decreases($m$ x)
  $E$[x,f]
}
\end{lstlisting}
\end{tabular}
\end{minipage}
%
\begin{minipage}{0.49\textwidth}
\begin{tabular}{c}
\begin{lstlisting}
$\lambda$x: $\tau_1$.
  rec[n $\Rightarrow \tarrow{x}{\trefine{x}{\tau_1}{\tapp{m}{x} < n}}{\tau_2}$](
    $\tsucc{\tapp{m}{x}}$,
    $\tlambda{x}{\trefine{x}{\tau_1}{\tapp{m}{x} < \tzero}}{\terr}$,
    $(n,f)\Rightarrow
      \tlambda{x}{\trefine{x}{\tau_1}{\tapp{m}{x} < \tsucc{n}}}{E[x,f \tu]}$
  ) x
\end{lstlisting}
\end{tabular}
\end{minipage}

\caption{Encoding of a function whose measure is given by the {\bf decreases}
  keyword (left) using the recursor (right). Both sides are expected to have
  type $\tarrow{x}{\tau_1}{\tau_2}$. On the right-hand-side, note that due to
  our definition of the recursor, we must write {\tt E[x,f $\tu$]} (and apply
  {\tt f} to $\tu$) to obtain a well-typed term.}
\label{fig:measure}

\end{figure}


==> figures/fig-plus_zero.tex <==
%! TEX root = ../main.tex

\begin{figure}[h]
  \hspace{-1em}\begin{minipage}{0.45\textwidth}
\begin{lstlisting}
def plus(x: Nat, y: Nat): Nat = x match {
  case $\tzero$ $\RA$ y
  case $\tsucc{z}$ $\RA$ $\tsucc{\tt plus(z, y)}$
}

def plus_zero(x: Nat): Unit = (x match {
  case $\tzero$ $\RA$ $\tu$
  case $\tsucc{y}$ $\RA$ plus_zero(y)
}) ensuring (res $\RA$ plus(x, $\tzero$) == x)
\end{lstlisting}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}
${\tt let}$ plus: $\tnat\rightarrow\tnat\rightarrow\tnat$ =
    $\lambda$x: $\tnat$. rec[$\cdots$]($\cdots$, $\cdots$, (n, plus) $\Rightarrow$
        $\lambda$x: $\tnat$. $\lambda$y: $\tnat$. ${\tt match}$(x, y, z $\RA$ plus () z y) x in

${\tt let}$ plus_zero: $\tarrow{x}{\tnat}{\trefine{u}{\tunit}{\tapp{\tapp{{\tt plus}}{x}}{\tzero}~{\tt ==}~x}}$ =
    $\lambda$x: $\tnat$. rec[$\cdots$]($\cdots$, $\cdots$, (n, plus_zero) $\Rightarrow$
        $\lambda$x: $\tnat$. ${\tt match}$(x, $\tu$, y $\RA$ plus_zero () y)) x
\end{lstlisting}
\end{minipage}
\caption{Desugaring of the functions \lstinline!plus! defining addition
on natural numbers and \lstinline!plus_zero! which states that
\lstinline!plus(n, $\tzero$) == n! and provides the inductive proof of
the property as its definition. We omit the measure functions and associated
refinements here for readability. }
\label{fig:plus_zero}
\end{figure}


==> figures/fig-pos.tex <==
%! TEX root = ../main.tex

\begin{figure}
\scriptsize
\begin{minipage}{0.49\textwidth}
\begin{flalign*}
  & \tpos{\alpha}{\tau} \define {\tt true} \textrm{ if $\alpha \not\in \fv{\tau}$}\\
  & \tpos{\alpha}{\alpha} \define {\tt true} \\
  & \tpos{\alpha}{\tarrow{x}{\tau_1}{\tau_2}} \define \tneg{\alpha}{\tau_1} \land \tpos{\alpha}{\tau_2} \\
  & \tpos{\alpha}{\tforall{x}{\tau_1}{\tau_2}} \define \tneg{\alpha}{\tau_1} \land \tpos{\alpha}{\tau_2} \\
  & \tpos{\alpha}{\tpoly{\beta}{\tau}} \define \tpos{\alpha}{\tau} \\
  & \tpos{\alpha}{\tsum{\tau_1}{\tau_2}} \define \tpos{\alpha}{\tau_1} \land \tpos{\alpha}{\tau_2} \\
  & \tpos{\alpha}{\tprod{x}{\tau_1}{\tau_2}} \define \tpos{\alpha}{\tau_1} \land \tpos{\alpha}{\tau_2} \\
  & \tpos{\alpha}{\indexedtype{n}{\beta}{\tau}} \define \tpos{\alpha}{\tau} \land (\alpha \notin \fv{\tau}\,\lor \tpos{\beta}{\tau}) \\
  & \tpos{\alpha}{\trefine{x}{\tau}{b}} \define \tpos{\alpha}{\tau}
\end{flalign*}
\end{minipage}
%
\begin{minipage}{0.49\textwidth}
\begin{flalign*}
  & \tneg{\alpha}{\tau} \define {\tt true} \textrm{ if $\alpha \not\in \fv{\tau}$}\\
  & \tneg{\alpha}{\alpha} \define {\tt false} \\
  & \tneg{\alpha}{\tarrow{x}{\tau_1}{\tau_2}} \define \tpos{\alpha}{\tau_1} \land \tneg{\alpha}{\tau_2} \\
  & \tneg{\alpha}{\tforall{x}{\tau_1}{\tau_2}} \define \tpos{\alpha}{\tau_2} \land \tneg{\alpha}{\tau_2} \\
  & \tneg{\alpha}{\tpoly{\beta}{\tau}} \define \tneg{\alpha}{\tau} \\
  & \tneg{\alpha}{\tsum{\tau_1}{\tau_2}} \define \tneg{\alpha}{\tau_1} \land \tneg{\alpha}{\tau_2} \\
  & \tneg{\alpha}{\tprod{x}{\tau_1}{\tau_2}} \define \tneg{\alpha}{\tau_1} \land \tneg{\alpha}{\tau_2} \\
  & \tneg{\alpha}{\indexedtype{n}{\beta}{\tau}} \define \tneg{\alpha}{\tau} \land (\alpha \notin \fv{\tau}\,\lor \tpos{\beta}{\tau}) \\
  & \tneg{\alpha}{\trefine{x}{\tau}{b}} \define \tneg{\alpha}{\tau}
\end{flalign*}
\end{minipage}

\caption{Definition of positivity and negativity for a type variable $\alpha$ in a type.}
\label{fig:pos}
\end{figure}


==> figures/fig-split.tex <==
%! TEX root = ../main.tex

\begin{figure}[htb]

\begin{lstlisting}
def split(l: List[$\tnat$], seps: List[$\tnat$]): List[List[$\tnat$]] = {
  l match {
    case Nil[$\tnat$] $\Rightarrow$ Cons(Nil[$\tnat$], Nil[List[$\tnat$]])
    case Cons(h, t) $\Rightarrow$
      if (contains(seps,h)) {
        Cons(Nil[$\tnat$], split(t, seps))
      } else {
        let r: List[List[$\tnat$]] = split(t, seps) in
        Cons(Cons(h, head(r), tail(r)))
      }
  } 
}
\end{lstlisting}

\caption{This function splits a list {\tt l} of natural numbers into a 
list of lists of natural numbers, by using the separators given {\tt seps} for
the cutting points.}
\label{fig:split}

\end{figure}

==> figures/fig-subalgo.tex <==

\begin{figure}
\[
\begin{array}{rcl}
  \subalgo{\Gamma}{\tau}{\tau}\\
  \subalgo{\Gamma}{\tarrow{x}{A}{B}}{\tarrow{x}{C}{D}} & \mathbf{if} & \subalgo{\Gamma}{C}{A}, \subalgo{\Gamma,x: A}{B}{D}\\
  \subalgo{\Gamma}{\tprod{x}{A}{B}}{\tprod{x}{C}{D}}   & \mathbf{if} & \subalgo{\Gamma}{A}{C}, \subalgo{\Gamma,x: A}{B}{D}\\
  \subalgo{\Gamma}{\tau}{\trefine{x}{A}{p}}            & \mathbf{if} & \areequal{\Gamma,x:\tau}{p}{\ttrue}\\
  \subalgo{\Gamma}{\trefine{x}{A}{p}}{\tau}            & \mathbf{if} & \subalgo{\Gamma}{A}{\tau}, \areequal{\Gamma,x: A}{p}{\ttrue}\\

\end{array}
\]
\caption{Algorithmic subtyping rules.
The rules are applied in the given order which leads to a
  deterministic subtyping relation. The rules concerning refinement
  subtyping generate \emph{verification conditions} by relying on the
  $\areequal{\Gamma}{p}{\ttrue}$ relation.}
\label{fig:subalgo}
\end{figure}


==> figures/fig-subtyping.tex <==
%! TEX root = ../main.tex

\begin{figure}

\seprules

\sidebyside
{
    \infer[\textit{(Subtype Refl)}]{
        \subtype{\Gamma}{\tau}{\tau}
    }{
        % \istype{\Gamma}{\tau}
    }
}
{
    \infer[\textit{(Subtype Trans)}]{
        \subtype{\Gamma}{\tau_1}{\tau_3}
    }{
        \subtype{\Gamma}{\tau_1}{\tau_2} &
        \subtype{\Gamma}{\tau_2}{\tau_3}
    }
}
 
% {
%     \infer[\textit{(Subtype Singleton)}]{
%         \subtype{\Gamma}{\tau}{\tlabsingleton{t}{\tau'}}
%     }{
%         \subtype{\Gamma}{\tau}{\tau'} &
%         \areequal{\Gamma, x: \tau}{x}{t}
%     }
% }

\seprules

% \ 
% {
%     \infer[\textit{(Subtype Arrow)}]{
%         \subtype{\Gamma}{\tarrow{x}{A_1}{B_1}}{\tarrow{x}{A_2}{B_2}}
%     }{
%         \subtype{\Gamma}{A_2}{A_1} &
%         \subtype{\Gamma, x: A_2}{B_1}{B_2}
%     }
% }

\ 
{
    \infer[\textit{(Subtype Arrow)}]{
        \subtype{\Gamma}{\tau}{\tarrow{x}{A}{B}}
    }{
        \hastype{\Gamma, f: \tau, a: A}{f\ a}{\subst{B}{x}{a}}
    }
}

\seprules

% \ 
% {
%     \infer[\textit{(Subtype Prod)}]{
%         \subtype{\Gamma}{\tprod{x}{A_1}{B_1}}{\tprod{x}{A_2}{B_2}}
%     }{
%         \subtype{\Gamma}{A_1}{A_2} &
%         \subtype{\Gamma, x: A_2}{B_1}{B_2}
%     }
% }

\ 
{
    \infer[\textit{(Subtype Prod)}]{
        \subtype{\Gamma}{\tau}{\tprod{x}{A}{B}}
    }{
        \hastype{\Gamma, p: \tau}{\tprojl{p}}{A} &
        \hastype{\Gamma, p: \tau}{\tprojr{p}}{\tletintype{x}{A}{\tprojl{p}}{B}}
    }
}

\seprules

\ 
{
    \infer[\textit{(Subtype Refine)}]{
        \subtype{\Gamma}{\tau}{\trefine{x}{A}{p}}
    }{
        \subtype{\Gamma}{\tau}{A} &
        \areequal{\Gamma, x: \tau}{p}{\ttrue}
    }
}
 
\seprules

\sidebyside
{
    \infer[\textit{(Subtype Generic)}]{
        \subtype{\Gamma}{\tau_1}{\tau_2}
    }{
        \hastype{\Gamma, x: \tau_1}{x}{\tau_2}
    }
}
{
    \infer[\textit{(Subtype Base)}]{
        \subtype{\Gamma}{\trefine{x}{A}{b}}{B}
    }{
        % \istype{\Gamma}{A} &
        \hastype{\Gamma, x: A, p: \tequal{b}{true}}{x}{B}
        % &
        % B \in \set{\tunit,\tbool,\tnat}
    }
}

\seprules

\ 
{
    \infer[\textit{(Subtype Let Step)}]{
        \subtype{\Gamma}
            {(\tletintype{x}{A}{t_1}{B})}
            {(\tletintype{x}{A}{t_2}{B})}
    }{
        \areequal{\Gamma}{t_1}{t_2}
    }
}

\seprules

\ 
{
    \infer[\textit{(Subtype Let Open 1)}]{
        \subtype{\Gamma}
            {(\tletintype{x}{A}{v}{B})}
            {\subst{B}{x}{v}}
    }{
        \hastype{\Gamma}{v}{A} &
        \isval{v}
    }
}

\seprules

\ 
{
    \infer[\textit{(Subtype Let Open 2)}]{
        \subtype{\Gamma}
            {\subst{B}{x}{v}}
            {(\tletintype{x}{A}{v}{B})}
    }{
        \hastype{\Gamma}{v}{A} &
        \isval{v}
    }
}

\seprules

% \ 
% {
%     \infer[\textit{(Subtype Let Open 2)}]{
%         \subtype{\Gamma}
%             {\subst{B}{x}{v}}
%             {(\tletintype{x}{A}{v}{B})}
%     }{
%         \hastype{\Gamma}{v}{A} &
%         \isval{v}
%     }
% }


% \seprules

% \ 
% {
%     \infer[\textit{(Subtype Base 2)}]{
%         \subtype{\Gamma}{\tlabsingleton{t}{A}}{B}
%     }{
%         \subtype{\Gamma}{A}{B} &
%         B \in \set{\tunit,\tbool,\tnat}
%     }
% }

% \sidebyside
% {
%     \infer[\textit{(Refine$_1$)}]{
%         \subtype{\Gamma}{\trefine{x}{A}{p}}{A}
%     }{
%         \istype{\Gamma}{A} &
%         \hastype{\Gamma, x: A}{p}{\tbool}
%     }
% }
% {
%     \infer[\textit{(Refine$_2$)}]{
%         \subtype{\Gamma}{\trefine{x}{A}{\ttrue}}{A}
%     }{
%         \istype{\Gamma}{A}
%     }
% }

% \seprules
 
% \ 
% {
%     \infer[\textit{(Refine$_3$)}]{
%         \subtype{\Gamma}{\trefine{x}{A}{p_1}}{\trefine{x}{B}{p_2}}
%     }{
%         \subtype{\Gamma}{A}{B} & 
%         \areequal{\Gamma, x: \trefine{x}{A}{p_1}}{p_2}{\ttrue}
%     }
% }

\caption{Subtyping rules. Symbols $\tau$, $\tau_1, \tau_2$, $A$, $B$ denote types}
\label{fig:subtyping}
\end{figure}


==> figures/fig-term-embedding.tex <==
%! TEX root = ../main.tex

\begin{figure}
\[
  \begin{array}{rclr}
    %\mbox{Term} & & \mbox{SMT Term} & \mbox{Assertions}\\
    \cembed{\tuerr}{\Theta;\Gamma} & = & x~~\mbox{fresh variable} & \neg\embed{\Theta;\Gamma} \\
    \cembed{\tapp{t_1}{t_2}}{\Theta;\Gamma} & = & \mathit{dispatch}_{\tau}(\cembed{t_1}{\Theta;\Gamma},\cembed{t_2}{\Theta;\Gamma}) & \emptyset \\
    \cembed{\tite{t_1}{t_2}{t_3}}{\Theta;\Gamma} & = & \mathit{ite}(\cembed{t_1}{\Theta;\Gamma}, \cembed{t_2}{\Theta;\Gamma,p:\tequal{t_1}{\ttrue}},\cembed{t_3}{\Theta;\Gamma,p:\tequal{t_1}{\tfalse}}) & \emptyset \\
    \cembed{\tmatch{t_n}{t_0}{n \Rightarrow t_s}}{\Theta;\Gamma} & = &
      \mathit{ite}(\cembed{t_n}{\Theta;\Gamma} \simeq \cembed{\tzero}{\Theta;\Gamma}, \cembed{t_0}{\Theta;\Gamma,p:\tequal{t_n}{\tzero}}, \cembed{t_s}{\Theta;\Gamma,n:\tnat,p:\tequal{t_n}{\tsucc{n}}}) & \emptyset \\
    \cembed{\tlambda{x}{\tau}{t}}{\Theta;\Gamma} & = & x~~\mbox{fresh variable} & \emptyset\\
  \end{array}
\]
\caption{Selection of term embedding rules.
  Embedding a term in our language
  produces both an SMT term and additional assertions (rightmost column).
  These are, for example, useful to ensure that evaluation cannot
  reach {\tt err} terms. For function applications, we rely on
  a $\mathit{dispatch}_{\tau}$ function indexed by the stripped
  type $\tau$ of the caller to ensure congruence.
  Lambda terms are conservatively replaced by fresh variables
  which constitutes a sound but imprecise approximation. }
  \label{fig:term-embedding}
\end{figure}


==> figures/fig-typeformation.tex <==
%! TEX root = ../main.tex

\begin{figure}[ht]

\sidebyside{
    \infer[\textit{(Form Unit)}]{
        \istype{\Gamma}{\tunit}
    }{
        \iscontext{\Gamma}
    }
}{
    \infer[\textit{(Form Bool)}]{
        \istype{\Gamma}{\tbool}
    }{
        \iscontext{\Gamma}
    }
}

\seprules

\sidebyside
{
    \infer[\textit{(Form Nat)}]{
        \istype{\Gamma}{\tnat}
    }{
        \iscontext{\Gamma}
    }
}
{
    \infer[\textit{(Form Arrow)}]{
        \istype{\Gamma}{\tarrow{x}{\tau_1}{\tau_2}}
    }{
        \istype{\Gamma}{\tau_1} &
        \istype{\Gamma, x: \tau_1}{\tau_2}
    }
}

\seprules

\
{
    \infer[\textit{(Form Pair)}]{
        \istype{\Gamma}{\tprod{x}{\tau_1}{\tau_2}}
    }{
        \istype{\Gamma}{\tau_1} &
        \istype{\Gamma, x: \tau_1}{\tau_2}
    }
}


\seprules

\
{
    \infer[\textit{(Form Refinement)}]{
        \istype{\Gamma}{\trefine{x}{\tau}{t}}
    }{
        \istype{\Gamma}{\tau} &
        \hastype{\Gamma, x: \tau}{t}{\tbool}
    }
}

\seprules

\
{
    \infer[\textit{(Form Identity)}]{
        \istype{\Gamma}{\tequal{t_1}{t_2}}
    }{
        \fv{t_1} \subseteq \sigdom(\Gamma) &
        \fv{t_2} \subseteq \sigdom(\Gamma)
    }
}
\seprules

\
{
    \infer[\textit{(Form Let)}]{
        \istype{\Gamma}{\tletintype{x}{t}{\tau_1}{\tau_2}}
    }{
        \hastype{\Gamma}{t}{\tau_1} &
        \istype{\Gamma, x: \tau_1, p{:}(\tequal{x}{t_1})}{\tau_2}
    }
}

\caption{Type formation rules}
\label{fig:typeformation}
\end{figure}


==> figures/fig-zipwith.tex <==
%! TEX root = ../main.tex

\begin{figure}
\begin{lstlisting}
def constant[X](x: X): @*\Stream{X}*@ = Stream(x, $\URA$ constant[X](x)))
\end{lstlisting}
\caption{Constant stream\label{fig:constant}}

\begin{lstlisting}

def zipWith[X,Y,Z](f: X $\RA$ Y $\RA$ Z, s1: @*\Stream{X}*@, s2: @*\Stream{Y}*@): @*\Stream{Z}*@ =
  Stream(f (@*\shead{s1}*@) (@*\shead{s2}*@), $\URA$ zipWith[X,Y,Z](f, @*\stail{s1},\ \stail{s2}*@) )
\end{lstlisting}
\caption{Zip function that combines elements of two streams using a two-argument function {\tt f}
\label{fig:zipwith}}

\begin{lstlisting}

def fib: $\Stream{\tbigint}$ = Stream(0, $\URA$ Stream(1, $\URA$ zipWith(plus, fib, @*\stail{fib}*@)))
\end{lstlisting}
\caption{Fibonacci stream defined using zipWith\label{fig:fibonacci}}
\end{figure}

==> fixpoint.tex <==
%! TEX root = main.tex

\begin{lstlisting}
def f(x: $\tau_1$): $\tau_2$ = {
  require($p$(x))
  decreases($m$(x))
  $E$[f]
}
\end{lstlisting}

$\tfix{\tarrow{x}{\tau_1}{\tau_2}}{x \Rightarrow m}{(f,x)\Rightarrow t_s}\ y$

$t_s[x/y,f/\tfix{\tarrow{x}{\tau_1}{\tau_2}}{x \Rightarrow m}{(f,x)\Rightarrow t_s}]$

%${\tt let}\ f: {\tarrow{x}{\tau_1}{\tau_2}}\ =\ \tfix{\tarrow{x}{\tau_1}{\tau_2}}{x \Rightarrow m}{f\Rightarrow t_s}\ {\tt in}\ t$

%$t[f/\tfix{\tarrow{x}{\tau_1}{\tau_2}}{x \Rightarrow m}{f\Rightarrow t_s}]$


\begin{multline*}
\begin{array}{ll}
\multicolumn{2}{l}{\lambda{x}: {\tau_1}.\ {rec[{n \Rightarrow \tarrow{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} < n}}{\tau_2}}]}(}\\
  & \tsucc{\tapp{m}{x}},\\
  & \tlambda{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} < \tzero}}{\terr},\\
  & (n,f)\Rightarrow \tlambda{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} \leq n}}{t_s})\ x
\end{array}
\end{multline*}

\begin{multline*}
\begin{array}{ll}
\multicolumn{2}{l}{(\lambda{x}: {\tau_1}.\ {rec[{n \Rightarrow \tarrow{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} < n}}{\tau_2}}]}(}\\
  & \tsucc{\tapp{m}{x}},\\
  & \tlambda{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} < \tzero}}{\terr},\\
  & (n,f)\Rightarrow \tlambda{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} \leq n}}{t_s})\ x)\ y
\end{array}
\end{multline*}

\begin{multline*}
\begin{array}{ll}
\multicolumn{2}{l}{{rec[{n \Rightarrow \tarrow{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} < n}}{\tau_2}}]}(}\\
  & \tsucc{\tapp{m}{y}},\\
  & \tlambda{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} < \tzero}}{\terr},\\
  & (n,f)\Rightarrow \tlambda{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} \leq n}}{t_s})\ y
\end{array}
\end{multline*}

\begin{multline*}
\begin{array}{ll}
\multicolumn{2}{l}{{rec[{n \Rightarrow \tarrow{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} < n}}{\tau_2}}]}(}\\
  & \tsucc{v},\\
  & \tlambda{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} < \tzero}}{\terr},\\
  & (n,f)\Rightarrow \tlambda{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} \leq n}}{t_s})\ y
\end{array}
\end{multline*}

\begin{multline*}
\begin{array}{ll}
\multicolumn{2}{l}{({\tt let}\ f: {\tarrow{x}{\tau_1}{\tau_2}}\ =\ {rec[{n \Rightarrow \tarrow{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} < n}}{\tau_2}}]}(}\\
  & v,\\
  & \tlambda{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} < \tzero}}{\terr},\\
  & (n,f)\Rightarrow \tlambda{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} \leq n}}{t_s})\ {\tt in}\\
\multicolumn{2}{l}{\tlambda{x}{\trefine{\_}{\tau_1}{\tapp{m}{x} \leq v}}{t_s[n/v]})\ y}
\end{array}
\end{multline*}

$\tlambda{x}{\trefine{\_}{\tau_1}{\tapp{m}{x}}}{t_s[n/v,f/g]})\ y$

$t_s[f/g,x/y]$




==> lists.tex <==
\input{figures/fig-lists}

\section{Definitions of Lists}

Figure~\ref{fig:lists} shows the definition of lists 
as an inductive data-type. The proofs can be extended in a straightforward by
defining the reducible values at type $\tlist{T}$ to be the terms of the form 
\(
  \tcons{T}{x_1}{\tcons{T}{x_2}{\dots\tcons{T}{x_n}{\tnil{T}}\dots}}
\)
with $n \geq 0$ and $x_1,\dots,x_n$ reducible values at type $T$. 


==> more-from-intro.tex <==
We now discuss different components of our system which contribute to its ease
of use, automation, and expressiveness.

Refinement types allow the user to give specification to functions in the same
programming language as pre and postconditions. The combination of refinement
and dependent types also give a natural way to give specification to
higher-order program, as in the following code snippet where function {\tt f},
which expects as argument a function {\tt g} which only returns values greater
than {\tt g}'s argument:

\begin{lstlisting}
def f(g: $\Pi$x :Nat. {y: Nat | y > x}) = // ...
\end{lstlisting}

To enforce termination of recursive functions, we use a type-based termination
technique that ensures that the type of the function in a recursive call is
strictly smaller than the type of the caller. Refinement types enables us to
define types that refer to user-defined or inferred measure functions that
ensure that recursive functions are terminating. Consequently, we can naturally
represent recursive functions with user-supplied (or inferred) measures
(including lexicographic measures) inside our terminating calculus. By using
type-based termination on recursive types indexed by natural numbers, we also
support termination arguments for recursive functions defined on infinite
data structures such as streams.

Another interesting aspect of our system is the use of (untyped) definitional
equality as a type. Equality types enable us to save the exact expression
(instead of just the type) of a let binding when type-checking, so that we can
verify assertions of the form:

\begin{lstlisting}
let a: BigInt = 5 in
assert(a == 5)
\end{lstlisting}

We also use equalities when defining recursive functions $f$. Typical typing
rules for recursive functions give access to the type of $f$ when type-checking
the body $E$ of $f$. Our typing rule allows in addition the body to be visible,
by remembering the equality $\tequal{f}{E}$ while type-checking $E$. This is
only possible with an untyped equality (an equality between terms that are not
necessarily well-typed), since we do not know yet whether $E$ is well-typed.
Therefore, user contracts that need to be checked within a recursive function
$f$ have access to the definition of $f$ itself. We show that this
\emph{body-visible recursion} (as opposed to simply \emph{type-visible}) feature
is sound and allows to reduce the notation overhead when verifying programs. A
similar feature is presented in \cite{DBLP:journals/pacmpl/VazouTCSNWJ18}.


%Equality is a fundamental aspect of logic and is a natural mechanism for 
%modeling recursive definitions.
%% System based on the notion of equality

%% Equalities
% The second part is about
% \emph{equalities} (identities) and the corresponding \emph{equality types}
% $\tequal{t_1}{t_2}$ over terms $t_1$ and $t_2$. Equalities denote a form of
% \emph{definitional equivalence} based on the call-by-value operational semantics
% of the language. Specifically, our system is built so that $\tequal{t_1}{t_2}$
% implies that $t_1$ and $t_2$ reduce to the same (syntactic) value in
% call-by-value operational semantics, or that they both diverge (we prove,
% however, that well-typed terms cannot diverge).

%% Equalities to express standard contracts
% We use equalities to express and verify user-written contracts. As an example,
% given an assertion or a pre-condition $b$ written by the user, we wish to check
% whether the equality $\tequal{\tt b}{\ttrue}$ holds at the point where the
% condition is required to hold. Furthermore, we use equalities to propagate
% information about let bindings $\tlet{x}{A}{t_1}{t_2}$, remembering that
% $\tequal{x}{t_1}$ holds when type-checking $t_2$.
%% Equalities are easy to think about
% Operational semantics of call-by-value systems are easy to understand for users.
% We therefore expect a system based on this definition of equality to be natural
% to use.

%%%%%%%%%%%%%%%%%%%%%%%%%
%% Proofs of identities do not carry computational content
%%%%%%%%%%%%%%%%%%%%%%%%%

% Our system uses a form of \emph{proof irrelevance} where the only term of type
% $\tequal{t_1}{t_2}$ is a dummy $\turefl$ term. The term $\turefl$ is a value of
% our language which does not carry computational content. This enables us not to
% worry about such proof terms when verifying properties related to operational
% semantics, and also use, for example, SMT solvers to establish them. We
% demonstrate the efficiency of our system by verifying a collection of
% higher-order functional programs.

%\subsection{Foundations of our Verification System}

% \subsection{Significance for Verification}

% This proof justifies the use of an approach
% that uses the same executable language to describe computation, specification,
% and termination measures.

%% Evaluation
% We present a verification system that is based on these foundations.
% To check the semantic side conditions that refer to operational semantics,
% our system makes an encoding of increasingly precise approximation
% of recursive functions using an SMT solver.

% Furthermore, we provide powerful inference mechanisms to automatically determine
% suitable measure functions, thus enabling natural writing of recursive programs
% with only minimal user annotation required for questions of termination
% (less than 10\% of recursive functions require measure annotation in our experience).

% \subsection{Contributions}


==> plus_zero-example.tex <==
%! TEX root = main.tex

\subsection{Type Checking Example}

\input{figures/fig-plus_zero}

Let us consider for example the definition and desugaring of the two recursive
functions presented in Figure~\ref{fig:plus_zero}.
The measure functions and associated refinements are
omitted in the example. The type checking rules defined in
Figure~\ref{fig:bidirectional} lead to a single verification condition
being generated in the $\tzero$ case of the \lstinline!plus_zero! {\tt match}
term (again omitting measure related conditions). Note that all other refinement
type checks go through by the \textit{(Check Reflexive)} rule.
We need to show that $(\tapp{\tapp{{\tt plus}}{x}}{\tzero} == x)\equiv\ttrue$
under the context given in Figure~\ref{fig:plus_zero-context}.

\begin{figure}[h]
\[
  \small
  \begin{array}{rcl}
    {\tt plus}       & : & \tnat\rightarrow\tnat\rightarrow\tnat,\\
    p\_plus          & : & \tequal{{\tt plus}}{\tlambda{x}{\tnat}{\tapp{\trec{\tnat\rightarrow\tnat\rightarrow\tnat}{\cdots}{\cdots}{\cdots}}{x}}},\\
    {\tt n}          & : & \tnat,\\
    {\tt plus\_zero} & : & \tunit\rightarrow\tarrow{x}{\tnat}{\trefine{u}{\tunit}{\tapp{\tapp{{\tt plus}}{x}}{\tzero}~{\tt ==}~x}},\\
    p\_plus\_zero    & : & \tequal{{\tt plus\_zero}}{\tlambda{u}{\tunit}{\trec{\tarrow{x}{\tnat}{\trefine{u}{\tunit}{\tapp{\tapp{\tt plus}{x}}{\tzero}~{\tt ==}~x}}}{\cdots}{\cdots}{\cdots}}},\\
    {\tt x}          & : & \tnat,\\
    p_0              & : & \tequal{\tt x}{\tzero}\\
    u                & : & \tunit\\
  \end{array}
\]
\caption{Context under which the equality
$(\tapp{\tapp{{\tt plus}}{x}}{\tzero} == x)\equiv\ttrue$ must be
  shown when type checking the program given in
  Figure~\ref{fig:plus_zero}.}
\label{fig:plus_zero-context}
\end{figure}

The initial embedding into SMT would not be sufficient to prove the
desired equivalence as we need to know that
$\tapp{\tapp{{\tt plus}}{\tzero}}{\tzero}\equiv\tzero$.
Recall that the ${\tt plus}$ lambda in the context will
be embedded into a fresh variable and its definition
therefore won't be available to the SMT solver.
However, after unfolding the body of
\lstinline!plus! (obtained from $p\_plus$), we can add
the equality type
$\tequal{\tapp{\tapp{{\tt plus}}{x}}{\tzero}}{\tmatch{x}{\tzero}{z \Rightarrow \tapp{\tapp{\tapp{{\tt plus}}{\tu}}{z}}{x}}}$
to the context and the SMT embedding becomes valid.


==> running-example2.tex <==
% %! TEX root = main.tex

% \section{Type-Checking Algorithm: Examples}
% \label{sec:motiv2}

% \itodo{Make sure to change these examples when we change the denotation of Rec(0)(\_).}

% \dtodo{We need rules for type-checking to $\ttop$.}


==> running-example3.tex <==
%! TEX root = main.tex

\section{Stream Examples: Type Generalization}
\label{sec:motiv3}

\subsection{Constant Stream}

We saw in Section~\ref{sec:motiv2} that our type-checker infers the type
$\tforall{n}{\tnat}{\tpoly{X}{X \Rightarrow \IStream{\tau}{n}}}$ for {\tt
constant}, but one might be interested in using {\tt constant} as a
\emph{normal} stream, i.e.~by checking that it has type $\tpoly{X}{X \Rightarrow
\Stream{\tau}}$:
\[
  \checktype
    {}
    {\tt constant}
    {\tpoly{X}{X \Rightarrow \Stream{\tau}}}.
\]

\subsection{ZipWith Function on Streams}

\subsection{Fibonacci Stream}


==> smt.tex <==
%! TEX root = main.tex

\subsection{Encoding Verification Conditions for SMT Solvers}
\label{sec:smt}

\input{figures/fig-term-embedding}
\input{figures/fig-context-embedding}

In order to discharge our verification conditions, we rely on two mutually
recursive embedding functions $\cembed{\cdot}{\Theta;\Gamma}$ from terms and
$\embed{\cdot}$ from typing contexts into a quantifier-free fragment of SMT.
The embedding is a sound over-approximation of our language semantics, namely if
$\embed{\Theta;\Gamma}\wedge\cembed{t_1}{\Theta;\Gamma}\not\simeq\cembed{t_2}{\Theta;\Gamma}$ is unsatisfiable, then
we know that $\areequal{\Theta;\Gamma}{t_1}{t_2}$ (however, satisfiability is only
sometimes indicative of an invalid equality). A selection of term embedding
and context embedding rules can be found in Figures~\ref{fig:term-embedding}
and \ref{fig:context-embedding}.

\ttodo{Embedding for recursive types?}

% We embed the $\tnat$ type into
% integers of the LIA theory with positivity constraints, and embed
% each $\tlist{\tau}$ type into the theory of inductive datatypes.
% A useful consequence of bidirectional type checking is that every sub-term
% within our program can be assigned a inferred type, which may include
% refinements. We leverage this to
% assert such refinements, thus strengthening the embedding into SMT. Concretely,
% during the embedding of $\cembed{t}{\Gamma}$, if we have
% $\checktype{\Gamma}{t}{\trefine{x}{\tau}{p}}$, then we produce the
% assertion $\embed{\Gamma}\implies\cembed{p}{\Gamma,x:\tau,p_x:\tequal{x}{t}}$.

% \dtodo{Reference to equality rules?.}

% We combine this embedding with an iterative procedure that
% alternates between checking validity of the embedded formula and performing
% term and context rewrites based on the equality rules defined in
% Figure~\ref{fig:equality} in order to improve the precision of the embedding.
% For example, the \textit{(Equal Destruct Nat 1)} rule enables us to
% \emph{unroll} {\tt rec} terms in our context in order to gain more information
% about their bodies.


==> soundness.tex <==
%! TEX root = main.tex

\section{Soundness of Our Type System}
\label{sec:soundness}

\subsection{Type Safety and Reducibility}
\label{sec:reducibility}

We prove in this section that any well-typed term $\hastype{\Gamma}{t}{\tau}$ is
\emph{reducible}, i.e.~$\redd{\Gamma}{t}{\tau}$. This statement also requires
proving properties on the subtyping and equality judgments. In particular, we
show that the equality judgment corresponds to the following notion of
equivalence: $\equivalent{t_1}{t_2}$ is defined to hold if for every value $v$,
$t_1 \smallstep^* v \iff t_2 \smallstep^* v$. Overall, we proved through mutual
induction on the typing, subtyping, and equality judgments the following facts.

\begin{restatable}{theorem}{reducible}
\label{th:reducible}
Given a context $\Gamma$, terms $t$, $t_1$, $t_2$, types $\tau$, $\tau_1$, $\tau_2$,
we have:
\begin{itemize}
\item $\hastype{\Gamma}{t}{\tau}$ implies $\redd{\Gamma}{t}{\tau}$, and
\item $\subtype{\Gamma}{\tau_1}{\tau_2}$ implies
$\forall \gamma \in \redvalues{\Gamma}{\interp}.\
    \redvalues{\gamma(\tau_1)}{\interp} \subseteq \redvalues{\gamma(\tau_2)}{\interp}$, and
\item $\areequal{\Gamma}{t_1}{t_2}$ implies
$\forall \gamma \in \redvalues{\Gamma}{\interp}. \equivalent{\gamma(t_1)}{\gamma(t_2)}$.
\end{itemize}
\end{restatable}

\begin{proof}
This proof has been carried out in the Coq proof assistant and covers
the core system as well as the extensions. We proceeded by
induction on the derivation of the judgments, or equivalently, on the height of
the derivation. Practically, for each typing, subtyping, or equality rule, we
assume that the theorem holds for the premises of the rule, and must deduce that
the theorem holds for the conclusion of the rule. We illustrate the proof on a
few rules. Some of the key lemmas that we use are referenced after the proof.

\begin{itemize}
\item Rule \textit{(Nat Intro 2)}. We know by induction hypothesis that
  $\redd{\Gamma}{e}{\tnat}$ and we must prove that
  $\redd{\Gamma}{\tsucc{e}}{\tnat}$.
  Equivalently, we need to show that given $\gamma \in \redvalues{\Gamma}{\interp}$,
  $\gamma(\tsucc{e}) \in \redexpr{\tnat}{\interp}$.

  Since $\redd{\Gamma}{e}{\tnat}$, we know that $\gamma(e) \in \redexpr{\tnat}{\interp}$,
  and by definition of $\redexpr{}{{\interp}}$ that there exists $v \in \redvalues{\tnat}{\interp}$
  such that $\gamma(e) \smallstep^* v$.

  We deduce from this and by definition of the operational semantics that
  $\gamma(\tsucc{e})$, which is equal to $\tsucc{\gamma(e)}$, reduces to
  $\tsucc{v}$, i.e.
  \[
    \gamma(\tsucc{e}) \smallstep^* \tsucc{v}
  \]
  By definition of $\redvalues{\tnat}{\interp}$, we have $\tsucc{v} \in
  \redvalues{\tnat}{\interp}$, which shows that $\gamma(\tsucc{e}) \in
  \redexpr{\tnat}{\interp}$. We can therefore conclude that
  $\redd{\Gamma}{\tsucc{e}}{\tnat}$.

\item Rule \textit{(Subsumption)}. We know by induction hypothesis that: (1)
  $\redd{\Gamma}{t}{\tau'}$ and (2) that for all $\gamma \in
  \redvalues{\Gamma}{\interp}$, we have $\redvalues{\gamma(\tau')}{\interp} \subseteq
  \redvalues{\gamma(\tau)}{\interp}$. We must conclude that $\redd{\Gamma}{t}{\tau}$.

  Let $\gamma \in \redvalues{\Gamma}{\interp}$. By (1), we know that $\gamma(t) \in
  \redexpr{\gamma(\tau')}{\interp}$. Therefore, there exists a value $v \in
  \redvalues{\gamma(\tau')}{\interp}$ such that $\gamma(\tau') \smallstep^* v$.
  From (2), we know that $v \in \redvalues{\gamma(\tau)}{\interp}$, and can conclude that
  $\gamma(t) \in \redexpr{\gamma(\tau)}{\interp}$, which is what we wanted to show.

\item Rule \textit{(Identity Intro)}. We know by induction hypothesis that for
  all $\gamma \in \redvalues{\Gamma}{\interp}$, we have
  $\equivalent{\gamma(t_1)}{\gamma(t_2)}$. We need to prove that
  $\redd{\Gamma}{\trefl}{\tequal{t_1}{t_2}}$. Let $\gamma \in
  \redvalues{\Gamma}{\interp}$. We must show that $\trefl \in
  \redexpr{\gamma(\tequal{t_1}{t_2})}{\interp}$, i.e.~$\trefl \in
  \redexpr{\tequal{\gamma(t_1)}{\gamma(t_2)}}{\interp}$, or equivalently that
  $\equivalent{\gamma(t_1)}{\gamma(t_2)}$, which is the case by assumption.

\item Rule \textit{(Arrow Elim)}.
  We know by induction hypothesis that:
  (1) $\redd{\Gamma}{t_1}{\tarrow{x}{\tau_2}{\tau}}$ and
  (2) $\redd{\Gamma}{t_2}{\tau_2}$.
  Our goal is to prove  that
    $\redd{\Gamma}{\tapp{t_1}{t_2}}{\tlet{x}{\tau_2}{t_2}{\tau}}$.
  Thus, we let $\gamma \in \redvalues{\Gamma}{\interp}$, and want to show
  that
    $\gamma(t_1\ t_2) \in
      \redexpr{\tlet{x}{\gamma(\tau_2)}{\gamma(t_2)}{\gamma(\tau)}}{\interp}$.

  By (2), we know that
    $\gamma(t_2) \in \redexpr{\gamma(\tau_2)}{\interp}$ and therefore that there exists
    a value $v \in \redvalues{\gamma(\tau_2)}{\interp}$ such that
    $\gamma(t_2) \smallstep^* v$.

  By (1), we know $\gamma(t_1) \in \redexpr{\tarrow{x}{\tau_2}{\tau}}{\interp}$, so there
  exists a value $f \in \redvalues{\tarrow{x}{\tau_2}{\tau}}{\interp}$ such that
  $\gamma(t_1) \smallstep^* f$.
  Moreover, by definition of $\redvalues{}{\interp}$ for the $\Pi$ type, we know that
  $f~v \in \redexpr{\subst{\gamma(\tau)}{x}{v}}{\interp}$. Then, since
  $\gamma(t_1~t_2) \smallstep^* f~v$, we deduce that
  $\gamma(t_1~t_2) \in \redexpr{\subst{\gamma(\tau)}{x}{v}}{\interp}$ as well.

  Finally, we have by Lemmas~\ref{lem:letstep} and \ref{lem:letopen} that
  $\redexpr{\tlet{x}{\gamma(\tau_2)}{\gamma(t_2)}{\gamma(\tau)}}{\interp} =
  \redexpr{\subst{\gamma(\tau)}{x}{v}}{\interp}$, which enables us to conclude that
    $\gamma(t_1\ t_2) \in
      \redexpr{\tlet{x}{\gamma(\tau_2)}{\gamma(t_2)}{\gamma(\tau)}}{\interp}$.

\item Rule \textit{(Equal Ite Eta)}
  We know by induction hypothesis that: (1)
  $\redd{\Gamma}{b}{\tbool}$, (2) for every
  $\gamma' \in \redvalues{\Gamma, x: \tequal{b}{\ttrue}}{\interp}$,
  $\equivalent{\gamma'(t_1)}{\gamma'(t)}$, and (3) for every
  $\gamma' \in \redvalues{\Gamma, x: \tequal{b}{\tfalse}}{\interp}$,
  $\equivalent{\gamma'(t_2)}{\gamma'(t)}$.

  Let $\gamma \in \redvalues{\Gamma}{\interp}$. We want to show:
  \[
    \equivalent{\tite{\gamma(b)}{\gamma(t_1)}{\gamma(t_2)}}{\gamma(t)}.
  \]
  By (1), we know that $\gamma(b) \smallstep^* \ttrue$ or
  $\gamma(b) \smallstep^* \tfalse$.

  Let us consider the case where $\gamma(b) \smallstep^* \ttrue$.
  This implies in particular that
  \[
    \equivalent{\tite{\gamma(b)}{\gamma(t_1)}{\gamma(t_2)}}{\gamma(t_1)}
     \qquad\qquad (4)
  \]

  Define $\gamma'$ to be the substitution $\gamma$ extended with the mapping $x
  \mapsto \trefl$. Since $\gamma(b) \smallstep^* \ttrue$, we deduce that $\trefl
  \in \redvalues{\tequal{\gamma(b)}{\ttrue}}{\interp}$ and therefore that $\gamma' \in
  \redvalues{\Gamma, x: \tequal{b}{\ttrue}}{\interp}$.

  By (2), we deduce that $\equivalent{\gamma'(t_1)}{\gamma'(t)}$. Moreover,
  since $x$ does not appear in $t_1$ nor in $t$, we have
  $\gamma'(t_1) = \gamma(t_1)$ and $\gamma'(t) = \gamma(t)$, meaning that
  $\equivalent{\gamma(t_1)}{\gamma(t)}$.
  By (4) and by transitivity of $\equivalent{}{}$, we conclude that:\qquad
  $\equivalent{\tite{\gamma(b)}{\gamma(t_1)}{\gamma(t_2)}}{\gamma(t)}$,
  which is what we wanted to show.


  The case where $\gamma(b) \smallstep^* \tfalse$ is treated in a symmetric way.


\end{itemize}

\end{proof}

\begin{lemma}
\label{lem:letstep}
Given terms $t_1$ and $t_2$ such that $t_1 \smallstep t_2$, and given types $A$
and $B$, we have:
\[
  \redvalues{\tletintype{x}{A}{t_1}{B}}{\interp} =
  \redvalues{\tletintype{x}{A}{t_2}{B}}{\interp}
\]
\end{lemma}

\begin{lemma}
\label{lem:letopen}
Given a value $v$ and types $A$, $B$, we have:
\[
  \redvalues{\tletintype{x}{A}{v}{B}}{\interp} =
  \redvalues{\subst{B}{x}{v}}{\interp}
\]
\end{lemma}


% A direct corollary of Theorem~\ref{th:reducible} is that

% \ttodo{Give some corollaries of soundness.}

We give two corollaries that follow from Theorem~\ref{th:reducible} and the
definition of $\redvalues{}{\interp}$. The first one states that any well-typed
term in an empty context does not crash, and normalizes to a value of the given
type.

\begin{corollary}
If $\hastype{}{t}{\tau}$, then there exists a value
$v \in \redvalues{\tau}{\interp}$ such that $t \smallstep^* v$.
\end{corollary}

The second corollary states that whenever we have a term $t$ whose type is a
refinement $\trefine{x}{A}{p}$, we can run the term $\tlet{x}{A}{t}{p}$ in
call-by-value semantics and obtain $\ttrue$. This holds for arbitrary
expressions $t$ and $p$, which can contain recursive functions.

\begin{corollary}
If $\hastype{}{t}{\trefine{x}{A}{p}}$, then there exists a value $v \in
\redvalues{A}{\interp}$ such that $t \smallstep^* v$ and $\subst{p}{x}{v}
\smallstep^* \ttrue$.
\end{corollary}



==> table.tex <==
\def\cm{\checkmark}
\begin{tabular}{|lrrrrlrr|}
  \hline
  Operation                  &  LoC & Funs & Rec Funs &          Measures & Annot. & Infer (s) & Check (s) \\
  \bname{Ackermann}          &   10 &    1 &        1 &             1 lex &      0 &       1.0 &       0.6 \\
  \bname{AliasPartial}       &   16 &    4 &        1 &             1 sum &      0 &       0.4 &       0.0 \\
  \bname{AmortizedQueue}     &  125 &   15 &        4 &             4 arg &      0 &       0.2 &       3.5 \\
  \bname{AnyDown}            &   21 &    1 &        1 &             1 lex &      0 &       0.8 &       0.0 \\
  \bname{AssociativeFold}    &  104 &   10 &        7 &             7 arg &      0 &       0.1 &       1.3 \\
  \bname{AssociativeList}    &   51 &    6 &        5 &             5 arg &      0 &       0.1 &       0.7 \\
  \bname{ChurchNum}          &   21 &    5 &        0 &                 - &        &         - &       0.0 \\
  \bname{CountTowardsZero}   &   16 &    1 &        1 &             1 sum &      0 &       0.3 &       0.5 \\
  \bname{EuclidGCD}          &  203 &   23 &        2 &             1 arg &      1 &       4.0 &       7.7 \\
  \bname{GodelNumbering}     &  420 &   46 &       25 &      2 sum/20 arg &      3 &      14.1 &      24.6 \\
  \bname{IndirectHO}         &   16 &    2 &        1 &             1 sum &      0 &       0.4 &       0.0 \\
  \bname{IndirectIntro}      &   24 &    3 &        2 &       1 lex/1 sum &      0 &       1.5 &       0.4 \\
  \bname{Indirect}           &   20 &    3 &        1 &             1 sum &      0 &       0.5 &       0.0 \\
  \bname{InsertionSort}      &   69 &    7 &        6 &       1 sum/5 arg &      0 &       0.7 &       0.9 \\
  \bname{Knapsack}           &   71 &    5 &        4 &       1 sum/2 arg &      1 &       1.4 &       0.5 \\
  \bname{ListMonad}          &   81 &   12 &        5 &       1 lex/4 arg &      0 &       3.5 &       1.2 \\
  \bname{ListOperations}     &  104 &   17 &        9 &       1 lex/8 arg &      0 &       6.5 &       1.1 \\
  \bname{List}               &  887 &   95 &       63 &      4 sum/59 arg &      0 &       4.9 &      10.6 \\
  \bname{McCarthy91}         &   24 &    2 &        1 &                 0 &      1 &         - &       0.7 \\
  \bname{MergeSorts}         &  199 &   21 &       17 &      4 sum/12 arg &      1 &       9.4 &       4.3 \\
  \bname{OddEvenComplex}     &   26 &    3 &        2 &                 0 &      2 &         - &       0.8 \\
  \bname{OddEvenMoreComplex} &   20 &    2 &        2 &                 0 &      2 &         - &       0.7 \\
  \bname{OddEven}            &   34 &    4 &        4 &             4 sum &      0 &       0.5 &       0.4 \\
  \bname{OptionMonad}        &   49 &    9 &        0 &                 - &        &         - &       0.7 \\
  \bname{QuickSorts}         &  219 &   25 &       15 &       5 sum/8 arg &      2 &      39.5 &      10.8 \\
  \bname{StableSort}         &  115 &   11 &        6 &       1 lex/5 arg &      0 &      20.7 &       2.0 \\
  \bname{ToChurch}           &   26 &    5 &        1 &             1 sum &      0 &       0.5 &       0.2 \\
  \bname{UpDown}             &   47 &    4 &        2 &             2 sum &      0 &       0.4 &       0.4 \\
  \bname{XPlus2N}            &   18 &    4 &        1 &             1 sum &      0 &       0.6 &       0.3 \\ \hline
  Total                      & 3036 &  346 &      189 &               174 &     13 &     112.0 &      74.9 \\ \hline
\end{tabular}



==> verifier.tex <==
%! TEX root = main.tex

\section{From System T with Refinements to Practice}
\label{sec:practice}

In this section we make a case that our type-checker
provides a useful basis for building a verifier for
higher-order functional programs with contracts.

We show how our verifier supports definitions that
use syntactically unconstrained recursion
by relying on measure functions. We discuss
how lexicographic measures can be handled
and provide a translation of such recursive
definitions into a combination of nested fixpoints and
refinement types that ensure that measures are decreasing.

% Using this notation we then explain the advantages of body-visible
% recursion that is supported in our system yet is not
% directly available in systems such as Coq (even with
% extensions such as Equations
% library~\cite{DBLP:conf/itp/Sozeau10}). Our typing rule
% provides soundness for such intuitive and flexible unfolding
% approach for reasoning about recursive functions.

